A Synchrotron Self-Compton Scenario for the Very High Energy Gamma-ray Emission of the Intermediate BL Lacertae object W Comae

W Comae has significant variability in multi-wavelengthes, from the radio to the gamma-ray bands. A bright outburst in the optical and X-ray bands was observed in 1998, and most recently, a strong TeV flare was detected by VERITAS in 2008. It is the first TeV intermediate-frequency-peaked BL Lacertae (IBL) source. I find that both the broadband spectral energy distributions (SEDs) quasi-simultaneously obtained during the TeV flare and during the optical/X-ray outburst are well fit by using a single-zone synchrotron + synchrotron-self-Compton (SSC) model. The satisfactory fitting requires a large beaming factor, i.e., $\delta\sim 25$ and $\delta\sim 20$ for the TeV flare and the optical/X-ray outburst, respectively, suggesting that both the optical/X-ray outburst and the TeV flare are from a relativistic jet. The size of the emission region of the TeV flare is three times larger than that of the optical/X-ray outburst, and the strength of the magnetic field for the TeV flare is $\sim 14$ times smaller than that of the X-ray/optical outburst, likely indicating that the region of the TeV flare is more distant from the core than that of the X-ray/optical outburst. The IC component of the TeV flare peaks at around 1.3 GeV, but it is around 20 MeV for the X-ray/optical outburst, lower than that for the TeV flare with 2 orders of magnitude. The model predicts that the optical/X-ray outburst might be accompanied by a strong MeV/GeV emission, but the TeV flare may be not associated with the X-ray/optical outburst. The GeV emission is critical to characterize the SEDs of the optical/X-ray outburst and the TeV flare. The predicted GeV flux is above the sensitivity of \emph{Fermi}/LAT, and it could be verified with the observations by \emph{Fermi}/LAT in near future.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
graphicx.sty   ---- a new package for embodying graphics, for LaTeX2e  
psfig.sty      ---- a package for graphics inclusion  
epsf.sty       ---- another package for graphics inclusion  
natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
f?.eps         ---- three demo figures used in the LaTeX template source

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

